Incentives for P2P-Assisted Content Distribution: If You Can't Beat 'Em, Join 'Em

The rapid growth of content distribution on the Internet has brought with it proportional increases in the costs of distributing content. Adding to distribution costs is the fact that digital content is easily duplicable, and hence can be shared in an illicit peer-to-peer (P2P) manner that generates no revenue for the content provider. In this paper, we study whether the content provider can recover lost revenue through a more innovative approach to distribution. In particular, we evaluate the benefits of a hybrid revenue-sharing system that combines a legitimate P2P swarm and a centralized client-server approach. We show how the revenue recovered by the content provider using a server-supported legitimate P2P swarm can exceed that of the monopolistic scheme by an order of magnitude. Our analytical results are obtained in a fluid model, and supported by stochastic simulations.

==> Conclusion.tex <==
\section{Conclusion}\label{s.conclusion}

Our goal in this paper is to quantify the ramifications of coopting legal P2P content sharing, not only as a means of reducing costs of content distribution, but, more importantly, as a way of hurting the performance of illegal P2P file sharing.  The model that we propose internalizes the idea that demand for any content is transient, and that all content will eventually be available for free through illegal file sharing.  The objective then is not to cling to ownership rights, but to extract as much revenue from legal copies as possible within the available time.  We develop a revenue sharing scheme that recognizes the importance of early adopters in extending the duration of time that revenue may be extracted.  In particular, keeping users from ``going rogue'' (becoming seeds in illegal networks) by allowing them to extract some revenue for themselves (and so defray part of their expense in purchasing the content in the first place), provides \emph{order sense improvements} in the extractable revenue.  We realize that our paradigm is contrary to the ``conventional wisdom'' of charging \emph{more} rather than \emph{less} to early adopters, and also to discourage file sharing using legal threats.  However, as many recent studies have demonstrated, incentives work better than threats in human society, and adoption of our revenue sharing approach might result in a cooperative equilibrium between content owners, distributors and end-users. Future work includes a characterization of the exact value of users based on their times of joining the system, as well as considering content streaming, which requires strict quality of service guarantees.  

==> Introduction.tex <==
\section{Introduction}
\IEEEPARstart{T}{he} past decade has seen the rapid increase of content distribution using the Internet as the medium of delivery  \cite{Lab09}.  Users and applications expect a low cost for content, but at the same time require high levels of quality of service.  However, providing content distribution at a low cost is challenging.  The major costs associated with meeting demand at a good quality of service are (i) the high cost of hosting services on the managed infrastructure of CDNs such as Akamai \cite{nor07,akamai}, and (ii) the lost revenue associated with the fact that digital content is easily duplicable, and hence can be shared in an illicit peer-to-peer (P2P) manner that generates no revenue for the content provider.  Together, these factors have led content distributors to search for methods of defraying costs.

One technique that is often suggested for defraying distribution costs is to use legal peer-to-peer (P2P) networks to supplement provider distribution \cite{pando,rawflow,RodTan06}.  It is well documented that the efficient use of P2P methods can result in significant cost reductions from the perspective of ISPs \cite{KarRod05,nor07}; however there are substantial drawbacks as well.  Probably the most troublesome is that providers fear losing control of content ownership, in the sense that they are no longer in control of the distribution of the content and worry about feeding illegal P2P activity.

Thus, a key question that must be answered before we can expect mainstream utilization of P2P approaches is: \emph{How can users that have obtained content legally be encouraged to reshare it legally?} Said in a different way, can mechanisms be designed that ensure legitimate P2P swarms will dominate the illicit P2P swarms?

In this paper, we investigate a ``revenue sharing'' approach to this issue.  We suggest that users can be motivated to reshare the content legally by allowing them to share the revenue associated with future sales.  This can be accomplished through either a lottery scheme or by simply sharing a fraction of the sale price.  Recent work on using lotteries to promote societally beneficial conduct \cite{MerPra09} suggests that such schemes could potentially see wide spread adoption.

Such an approach has two key benefits:  First, obviously, this mechanism ensures that users are incentivized to join the legitimate P2P network since they can profit from joining.  Second, less obviously, this approach actually damages the illicit P2P network.  Specifically, despite the fact that content is free in the illicit P2P network, since most users expect a reasonable quality of service, if the delay in the illegitimate swarm is large they may be willing to use the legitimate P2P network instead.  Thus, by encouraging users to reshare legitimately, we are averting them from joining the illicit P2P network, reducing its capacity and performance; thus making it less likely for others to use it.

The natural concern about a revenue sharing approach is that by sharing profits with users, the provider is losing revenue. However, the key insight provided by the results in this paper is that by discouraging users from joining illicit P2P network, the increased share (possibly exponentially more) of legitimate copies makes up for the cost of sharing revenue with end-users.

%is that the bootstrapping provided by the second effect described above provides a magnification of the initial revenue sharing ``investments'', which turns out to provide exponential gains in revenue for the provider even when very little revenue sharing is used.

More specifically, the contribution of this paper is to develop and analyze a model to explore the revenue sharing approach described above.  Our model (see Section \ref{s.model}) is a fluid model that builds on work studying the capacity of P2P content distribution systems.  The key novel component of the model is the competition for users among an illicit P2P system and a legal content distribution network (CDN), which may make use of a supplementary P2P network with revenue sharing. The main results of the paper (see Section \ref{s.results}) are Theorems~\ref{thm:inefficient}-\ref{thm:efficient-bass}, which highlight the order-of-magnitude gains in revenue extracted by the provider as a result of participating in revenue sharing.  Further, %Corollary \ref{c.epsiloninefficient} highlights that the optimal amount of revenue sharing is quite small.  
In addition to the analytic results, to validate the insights provided by our asymptotic analysis of the fluid model we also perform numerical experiments of the underlying finite stochastic model.  Tables \ref{tbl:ineff} and \ref{tbl:eff} summarize these experiments, which highlight both that the results obtained in the fluid model are quite predictive for the finite setting and that there are significant beneficial effects of revenue sharing.  %In particular, the examples that we present indicate that revenue extraction gains between $25\%$ to $180\%$ are possible through appropriate revenue sharing.

There is a significant body of prior work modeling and analyzing P2P systems.  Perhaps the most related work from this literature is the work that focuses on server-assisted P2P content distribution networks \cite{WanYeo07,SetApo07,LiuZha08,ChePon08,ShaJoh10,ParSha11A} in which a central server is used to ``boost'' P2P systems.  This boost is important since pure P2P systems suffer poor performance during initial stages of content distribution.  In fact, it is this initially poor performance that our revenue sharing mechanism exploits to ensure that the legitimate P2P network dominates.

Two key differentiating factors of the current work compared to this work are:  (i) We model the impact of competition between legal and illegal swarms on the revenue extraction of a content provider.   (ii) Unlike most previous works on P2P systems, we consider a time varying viral demand model for the evolution of demand in a piece of content based on the Bass diffusion model (see Section \ref{s.model}). Thus, we model the fact that interest in content grows as interested users contact others and make them interested.


With respect to (i), there has been prior work that focuses on identifying the relative value of content and resources for different users \cite{gamenets,MisIon10}.  For instance, \cite{gamenets} deals with creating a content exchange that goes beyond traditional P2P barter schemes, while \cite{MisIon10} attempts to characterize the relative value of peers in terms of their impact on system performance as a function of time.   However, to the best of our knowledge, ours is the first work that considers the question of economics and incentives in hybrid P2P content distribution networks.  

With respect to (ii), there has been prior work that considers fluid models of P2P systems such as \cite{QiuSri04,MasVoj05,YanVec06}.  However, these all focus on the performance evaluation of a P2P system with constant demand rate.  As mentioned above, a unique facet of our approach is that we explicitly make use the transient nature of demand in our modeling.  In the sense of explicitly accounting for transient demand, the closest work to ours is \cite{ShaJoh10}.  However, \cite{ShaJoh10} focuses only on jointly optimizing server and P2P usage in the case of transient demand in order to obtain a target delay guarantee at the lowest possible server cost.

The remainder of the paper is organized as follows.  We first introduce the details of our model in Section \ref{s.model}.  Then, Section \ref{s.results} summarizes analytic and numeric results, the proofs of which are included in the appendix.  Finally, Section \ref{s.conclusion} provides concluding remarks.




